LoMOE: Localized Multi-Object Editing via Multi-Diffusion

Recent developments in the field of diffusion models have demonstrated an exceptional capacity to generate high-quality prompt-conditioned image edits. Nevertheless, previous approaches have primarily relied on textual prompts for image editing, which tend to be less effective when making precise edits to specific objects or fine-grained regions within a scene containing single/multiple objects. We introduce a novel framework for zero-shot localized multi-object editing through a multi-diffusion process to overcome this challenge. This framework empowers users to perform various operations on objects within an image, such as adding, replacing, or editing $\textbf{many}$ objects in a complex scene $\textbf{in one pass}$. Our approach leverages foreground masks and corresponding simple text prompts that exert localized influences on the target regions resulting in high-fidelity image editing. A combination of cross-attention and background preservation losses within the latent space ensures that the characteristics of the object being edited are preserved while simultaneously achieving a high-quality, seamless reconstruction of the background with fewer artifacts compared to the current methods. We also curate and release a dataset dedicated to multi-object editing, named $\texttt{LoMOE}$-Bench. Our experiments against existing state-of-the-art methods demonstrate the improved effectiveness of our approach in terms of both image editing quality and inference speed.

==> sections/tabs/full_ablation.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{cccccccccc}
        \toprule
        $\mathcal{L}_{xa}$ & $\mathcal{L}_{b}$ & $\tau$ & $T_b$ & \makecell{Source CLIP\\Score ($\uparrow$)} & \makecell{Background\\LPIPS ($\downarrow$)} & \makecell{Background\\PSNR ($\uparrow$)}  & \makecell{Background\\SSIM ($\uparrow$)} & \makecell{Structural\\Distance ($\downarrow$)} & \makecell{Target CLIP\\Score ($\uparrow$)}\\
        \midrule
        \xmark & \xmark & - & - & 23.0906 & 0.1088 & 26.4474 & 0.8537 & 0.0763 & 26.2555\\
        \xmark & \cmark & - & - &  23.3925 & 0.0554 & 30.1475 & 0.8818 & 0.0728 & \textbf{26.2662}\\
        \cmark & \xmark & - & - &  \textbf{23.6611} & 0.0749 & 26.9587 & 0.8698 & 0.0699 & 26.1338\\
        \cmark & \cmark & - & - &  23.5445 & \textbf{0.0546} & \textbf{30.3154} & \textbf{0.8847} & \textbf{0.0661} & 26.0740\\
        \midrule
        - & - & 1.00 & - & 23.4216 & 0.0586 & 30.1023 & 0.8822 & 0.0728 & 25.9163\\
        - & - & 1.25 & - & \textbf{23.7507} & 0.0522 & 30.4707 & 0.8849 & 0.0715 & \textbf{26.0902}\\
        - & - & 1.50 & - & 24.1785 & 0.0497 & 30.7565 & 0.8863 & 0.0708 & 25.7919\\
        - & - & 1.75 & - & 25.0428 & 0.0466 & 31.1206 & 0.8875 & 0.0709 & 24.9769\\
        - & - & 2.00 & - & 25.4275 & \textbf{0.0409} & \textbf{31.5829} & \textbf{0.8896} & \textbf{0.0652} & 24.1544\\
        \midrule
        - & - & - & 05 & 23.5422 & 0.0562 & 30.1123 & 0.8838 & 0.0782 & 25.9403\\
        - & - & - & 10 & \textbf{23.5445} & \textbf{0.0546} & \textbf{30.3154} & \textbf{0.8847} & \textbf{0.0710} & \textbf{26.0740}\\
        - & - & - & 20 & 23.4344 & 0.0587 & 30.0937 & 0.8822 & 0.0723 & 25.8746\\
        - & - & - & 30 & 23.4494 & 0.0618 & 29.8495 & 0.8792 & 0.0757 & 25.9404\\
        - & - & - & 35 & 23.2644 & 0.0621 & 29.8123 & 0.8792 & 0.0774 & 25.8089\\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:ablation-experiments} ablation experiments}
\end{table*}
